Optimizing Cursor Loops in Relational Databases

Loops that iterate over SQL query results are quite common, both in application programs that run outside the DBMS, as well as User Defined Functions (UDFs) and stored procedures that run within the DBMS. It can be argued that set-oriented operations are more efficient and should be preferred over iteration; but from real-world use cases, it is clear that loops over query results are inevitable in many situations, and are preferred by many users. Such loops, known as cursor loops, come with huge trade-offs and overheads w.r.t. performance, resource consumption and concurrency. We present Aggify, a technique for optimizing loops over query results that overcomes all these overheads. It achieves this by automatically generating custom aggregates that are equivalent in semantics to the loop. Thereby, Aggify completely eliminates the loop by rewriting the query to use this generated aggregate. This technique has several advantages such as: (i) pipelining of entire cursor loop operations instead of materialization, (ii) pushing down loop computation from the application layer into the DBMS, closer to the data, (iii) leveraging existing work on optimization of aggregate functions, resulting in efficient query plans. We describe the technique underlying Aggify and present our experimental evaluation over benchmarks as well as real workloads that demonstrate the significant benefits of this technique.

==> response.tex <==
%\cleardoublepage
\clearpage
\newcommand{\itemit}[1]{\item \textit{{#1}}}
\newcommand{\itemitt}[2]{\item[{#1}] \textit{{#2}}}

\section*{Response to Reviewer Comments}
We would like to acknowledge the Reviewers and Meta Re-
viewer for their valuable comments and suggestions.

\subsection*{Meta-Review Comments}
\textit{At a high level, the main concerns to be addressed are: \\
1) including a more standardized approach to the experiments, as well as a more precise language model/extraction algorithm, and \\
2) more evidence that the workloads chosen for the experiments are representative of loops in the wild. One way to do this would be to include some of the loops you looked at in the experiment pool. More specifically,
(a) The experimental evaluation needs to be adjusted as suggested in R1's D4/D5 and R3's W1
(b) The loops discussed in the author feedback ("We have manually looked at many such loops, and our modification of TPC\-H is inspired by these") should be added to the experiment pool.\\}


\noindent\textbf{Response.} We trust we have addressed these concerns, as summarized in major changes below.
 
\subsection*{Summary of Major Changes}

\begin{enumerate}%[leftmargin=*,noitemsep]
  \item

  \item

  \item

  \item
\end{enumerate}
Note: Major additions and modifications have been highlighted in \textcolor{blue}{blue} in the paper.

\subsection*{Reviewer 1 Comments}
\begin{enumerate} %[leftmargin=*,noitemsep]

\itemit{R1\_W1: The aggregate extraction algorithm is underspecified.}
  
\textbf{Response.} 

\itemit{R1\_W2:  Experiments are somewhat ad-hoc.}
  
\textbf{Response.} 

\itemit{R1\_W3: The paper is written, at least in part, for a PL audience.}
  
\textbf{Response.} 
\end{enumerate}

\section*{Reviewer 2 Comments}

\begin{enumerate}% [leftmargin=*,noitemsep]
	
	
\itemit{R2\_W1: Weak evaluation.}
 
\textbf{Response.} 
 

\itemit{R2\_D: Applicability of the proposed technique.}
 
\textbf{Response.} 
\end{enumerate}

 
\section*{Reviewer 3 Comments}

\begin{enumerate} %[leftmargin=*,noitemsep]
	
	
\itemit{R3\_W1: In the experimental evaluation, multiple things are varied across different experiments. In one experiment, only Aggify is shown, in another one Aggify+Froid. Scaling is shown for a workload that has not been evaluated before. It would have been better to evaluate the method in a consistent fashion under different properties and each property for all workloads. Besides, more details on the real-world workload would be beneficial.}
 
\textbf{Response.}


\itemit{R3\_W2: I wonder how present the excessive use of cursors really still is in practice and whether the authors solve a real problem here. The paper cites only a blog post on that topic from 2015 to motivate the need for their technique. Furthermore, if using cursors is a bad habit, then this technique enforces users to stick to these habits even more.}

\textbf{Response.} 


\itemit{R3\_W3: The method is a pretty straight-forward template replacement technique. While simplicity is good for practicability and robustness, the overall research contribution is relatively limited.}

\textbf{Response.} .

\end{enumerate}


